Large Language Model Should Understand Pinyin for Chinese ASR Error Correction

Large language models can enhance automatic speech recognition systems through generative error correction. In this paper, we propose Pinyin-enhanced GEC, which leverages Pinyi, the phonetic representation of Mandarin Chinese, as supplementary information to improve Chinese ASR error correction. Our approach only utilizes synthetic errors for training and employs the one-best hypothesis during inference. Additionally, we introduce a multitask training approach involving conversion tasks between Pinyin and text to align their feature spaces. Experiments on the Aishell-1 and the Common Voice datasets demonstrate that our approach consistently outperforms GEC with text-only input. More importantly, we provide intuitive explanations for the effectiveness of PY-GEC and multitask training from two aspects: 1) increased attention weight on Pinyin features; and 2) aligned feature space between Pinyin and text hidden states.

==> sections/4-result.tex <==
\section{Experimental Results}

\subsection{Results for PY-GEC}


In Table~\ref{table:asr1}, we observe consistent improvements in CERs and entity recalls across all test sets using LLM-based correction methods. Specifically, direct correction enhances the average CER and entity recall from 13.43\% and 64.95\% to 11.48\% and 70.19\%, respectively. Furthermore, the PY-GEC method achieves even better performance, with a CER of 11.10\% and an entity recall of 70.82\%. Notably, when using multitask training and PY-GEC, we achieve the lowest CER and the highest entity recall across all ASR models and test sets. The average CER and entity recall reach 10.53\% and 72.93\%, respectively, proving the effectiveness of our proposed approach. Analyzing Figure~\ref{fig:bar}, we find that on the Aishell dataset, multitask training and PY-GEC significantly improve the percentage of good cases from 18.66\% to 28.57\%, while reducing bad cases from 6.42\% to 5.39\%. On the Common Voice dataset, the percentage of good cases increases from 38.52\% to 45.53\%, while bad cases remain relatively stable.

After multitask training, the LLM can perform direct correction with text-only input and re-transcription from Pinyin-only input. Surprisingly, when using multitask training, direct correction performs comparably to PY-GEC and outperforms direct correction without multitask training. This suggests that multitask training enhances the LLM’s internal understanding of input text's pronunciation, improving its ability to recognize and correct ASR errors. Furthermore, retranscription can improve the ASR performance of the Whisper-Small model but not the Whisper-Large model.

Ensembling results from the multitask-trained LLM is generally effective. However, the traditional sequence merging method, ROVER, does not enhance the CER or entity recall. In contrast, the Pinyin-Rerank method consistently improves both CER and entity recall across all setups. Although LLM-Rerank achieves the highest entity recall, its CER is higher than that of Pinyin-Rerank and requires more computational resources.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/bar.jpg}
  \caption{The percentages of good and bad cases. The ASR transcriptions are generated by Whisper-Small on Aishell-1 and Common Voice datasets.}
  \label{fig:bar}
\end{figure}

\subsection{Attention Analysis}

The attention scores depicted in Figure~\ref{fig:att} shed light on the significance of each input component in the error correction process. Notably, for the naive PY-GEC approach, Pinyin exerts a more substantial influence than the input hypothesis. However, it is the prediction that receives the highest attention score. This observation suggests that the GEC process predominantly relies on the context provided by nearby output tokens. Multitask training enhances the importance of Pinyin features, as indicated by the highest attention score, demonstrating that the LLM better comprehends Pinyin features.

Figure~\ref{fig:att_layer} illustrates the layer-wise attention scores. For PY-GEC, we observe that the importance of each component remains similar across the initial 24 layers. However, as we delve deeper into the network, the predicted tokens receive increased attention. In the multitask training scenario, Pinyin features consistently exhibit higher attention scores across all layers compared to the features of the hypothesis, while predicted tokens continue to play a crucial role at deeper layers

\begin{figure}[t]
  \centering
  \includegraphics[width=0.6\linewidth]{figures/att.jpg}
  \caption{The attention scores correspond to each input component.}
  \label{fig:att}
\end{figure}


\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/layer_att.jpg}
  \caption{The layer-wise attention scores correspond to each input component. (a) PY-GEC; (b) Multitask + PY-GEC.}
  \label{fig:att_layer}
\end{figure}

\subsection{Feature Space Analysis}

In Table~\ref{table:sim}, we evaluate the alignment between text and Pinyin, as outlined in section~\ref{sec:align}. Initially, without fine-tuning, the LLaMA-3-8B-Chinese shows poor alignment with a low cosine similarity of 0.26. Fine-tuning with PY-GEC or multitask training can both significantly boost the alignment with cosine similarity improved to 0.74 and 0.82 respectively. These results also verify the benefits of incorporating conversion tasks to enhance text-Pinyin alignment. Unexpectedly, even the model fine-tuned with direct correction demonstrates better text-Pinyin alignment. Despite not having been exposed to Pinyin features during training, this model likely learns Chinese character pronunciation from the ASR correction task, closing the gap between text and Pinyin. This further emphasizes the importance of promoting phonetic representation understanding within large language models for better correction performance.

Figure~\ref{fig:pca} illustrates the feature space of text and Pinyin. In Figure~\ref{fig:pca} (a), we observe that our approach (multitask + PY-GEC) brings the feature space between text and Pinyin much closer than the original LLM. However, text and Pinyin still occupy distinct feature spaces, indicating that the LLM perceives semantic and phonetic information differently. Further analysis of higher-dimensional feature spaces (Figure~\ref{fig:pca} (b, c)) reveals that the original LLM places text samples in sparser regions compared to Pinyin samples. In contrast, our fine-tuned model exhibits similar spatial distributions for text and Pinyin, with clusters showing comparable shapes except for the first principal component.

\begin{table}[t]
\caption{The cosine similarity between the text and the Pinyin vectors.}
\small
\centering
\begin{tabular}{c | c} 
\toprule
& cosine similarity \\
\midrule
LLaMA-3-8B-Chinese & 0.26\\
Direct & 0.45 \\
PY-GEC & 0.74\\
\textbf{Multitask + PY-GEC} & \textbf{0.82}\\
\bottomrule
\end{tabular}

\label{table:sim}
\end{table}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/pca.jpg}
  \caption{PCA analysis for the last hidden states that correspond to Text and Pinyin. The hidden states are extracted from the original LLaMA-3-8B-Chinese model and our fine-tuned multitask model.}
  \label{fig:pca}
\end{figure}


% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=0.65\linewidth]{figures/sim.jpg}
%   \caption{The cosine similarity matrices between the hidden states of text tokens and hidden states of Pinyin tokens.}
%   \label{fig:sim}
% \end{figure}
